Exploring Programming Task Creation of Primary School Teachers in Training

Introducing computational thinking in primary school curricula implies that teachers have to prepare appropriate lesson material. Typically this includes creating programming tasks, which may overwhelm primary school teachers with lacking programming subject knowledge. Inadequate resulting example code may negatively affect learning, and students might adopt bad programming habits or misconceptions. To avoid this problem, automated program analysis tools have the potential to help scaffolding task creation processes. For example, static program analysis tools can automatically detect both good and bad code patterns, and provide hints on improving the code. To explore how teachers generally proceed when creating programming tasks, whether tool support can help, and how it is perceived by teachers, we performed a pre-study with 26 and a main study with 59 teachers in training and the LitterBox static analysis tool for Scratch. We find that teachers in training (1) often start with brainstorming thematic ideas rather than setting learning objectives, (2) write code before the task text, (3) give more hints in their task texts and create fewer bugs when supported by LitterBox, and (4) mention both positive aspects of the tool and suggestions for improvement. These findings provide an improved understanding of how to inform teacher training with respect to support needed by teachers when creating programming tasks.

==> tables/generalCategories.tex <==
\begin{table}[t]\centering
	\caption{Reflection of \teachersintraining about further needed support when creating a task. 
	% \\ \textmd{The percentage refers to the proportion of \teachersintraining mentioning the (sub-)category at least once.}
 }
	\vspace{-1em}
	\label{tab:general}
	%\setlength{\tabcolsep}{0.2em}
	%\resizebox{\columnwidth}{!}{
\begin{tabular}{lrllllll}
    \toprule
	(Sub-)Category & \multicolumn{2}{l}{\% \teachersintraining} \\
 
	\midrule

    \rowcolor{Gray} Simplicities & \percentagegeneralReflectionsimplicities \% & \DrawPercentageBar{\percentagegeneralReflectionsimplicities} \\

    \hspace{0.5em} general & \percentagegeneralReflectionsimplicitiesgeneral \% & \DrawPercentageBar{\percentagegeneralReflectionsimplicitiesgeneral} \\

    \hspace{0.5em} use of simplification material & \percentagegeneralReflectionsimplicitiessimplificationthrough \% & \DrawPercentageBar{\percentagegeneralReflectionsimplicitiessimplificationthrough} \\
    \hspace{0.5em} programming &  \percentagegeneralReflectionsimplicitiesprogramming\% & \DrawPercentageBar{\percentagegeneralReflectionsimplicitiesprogramming} \\
    % \hspace{0.5em} sprites and backgrounds & \percentagegeneralReflectionsimplicitiesdealingwithspritesandorbackground \% & \DrawPercentageBar{\percentagegeneralReflectionsimplicitiesdealingwithspritesandorbackground} \\

    \rowcolor{Gray} Difficulties & \percentagegeneralReflectiondifficulties \% & \DrawPercentageBar{\percentagegeneralReflectiondifficulties} \\
    \hspace{0.5em} programming & \percentagegeneralReflectiondifficultiesprogramming \% & \DrawPercentageBar{\percentagegeneralReflectiondifficultiesprogramming} \\
    \hspace{0.5em} non-technical problems & \percentagegeneralReflectiondifficultiesnontechnicalproblems \% & \DrawPercentageBar{\percentagegeneralReflectiondifficultiesnontechnicalproblems} \\

\bottomrule
\end{tabular}
%}
\end{table}
